Time-domain and Frequency-domain Signals and their Analysis

Depending on the application people use time-domain or frequency-domain signals in order to measure or describe processes. First we will look at the definition of these terms, produce some mathematical background and then apply the tools to measurements made in the accelerator domain. We will first look at signals produced by a single bunch passing once through a detector (transfer line, linac), then periodic single bunch passages (circular accelerator) and at the end multi-bunch passages in a circular accelerator.

==> debris1.tex <==
\subsubsection{Fourier transform of a longitudinally Gaussian shaped beam}
\vspace{8mm}
\begin{importantbox}
The Fourier transform of a Gaussian-shaped longitudinal particle distribution in time-domain is also a Gaussian-shaped function in frequency-domain (see \Fref{fig:TFD-specgauss}). Again, since negative frequencies have no physical meaning, we only use the right side of the curve as spectral information.
The width of the frequency spectrum is proportional to the inverse of the bunch-length. Hence \textbf{shorter bunches} have a \textbf{wider spectrum}, which means they contain frequency components of higher frequency than longer bunches. 
\label{box:TFD-bulength}
\end{importantbox}

\begin{wrapfigure}[7]{R}{0.5\textwidth}
  \begin{center}
  \includegraphics[width=0.45\textwidth]{TFD-figures/Picture10}
  \end{center}
\caption{Spectrum (red) of a Gaussian-shaped time domain function (blue). The widths of the distributions are inversely proportional.}
  \label{fig:TFD-specgauss}
\end{wrapfigure}
\noindent At low beam energies the longitudinal shape is determined by the particle source and by the choice of the first accelerating system. The shapes can be quite different.
With increasing energy an several successive accelerating elements, the longitudinal bunch shape gets more regular and can often be approximated by a Gaussian distribution.




Much more details on longitudinal bunch shapes and the corresponding frequency spectra are treated in \Sref{sec:bulen}.

\newpage

\subsection{Analog Digital Conversion Basics}

We will use in many locations the term \textbf{Analog Digital Conversion (ADC)}. What we mean is the measurement of the instantaneous amplitude of an input signal at regular intervals $\Delta t$ and a final representation of this measurement as digital information.
A very detailed description of the techniques and of related phenomena can be found in \cite{bib:TFD-Gasior1}. 
\begin{figure}[!ht]
  \begin{center}
    \includegraphics[width=0.7\textwidth]{TFD-figures/Picture19}
 	\end{center}
  	\caption{Illustration of the analog - digital conversion of a sine wave}
    \label{fig:TFD-ADC}
\end{figure}
\Fref[b]{fig:TFD-ADC} illustrates the process of the analog digital conversion. The green trace is the continuous input signal, the red curve the input signal measured with a very coarse quantization value $q$ and the blue curve shows the difference, which we usually refer to as quantization error.

The following list gives definitions of terms used in this context:
\begin{enumerate}
\item{ \begin{itemize}
		\item{ A: input signal amplitude}
		\item{ n: number of bits}
		\item{ $q$: one bit amplitude; $q  = \frac{2A}{2^n}$}
		\end{itemize}
		}
\item{Maximum quantization error: $e_m = \frac{\pm q}{2}$
}
\item{RMS amplitude of the input signal $A_{RMS} =\frac{A}{\sqrt{2}}$
}
\item{Quantization error RMS amplitude: $e_{RMS} = \frac{1}{\sqrt{12}}q \simeq 0.289 q$
}
\item{Signal to Noise Ratio: $SNR:=\frac{A_{RMS}}{e_{RMS}} = \frac{\sqrt{6}}{2}2^n$
}
\item{Signal to Noise Ratio [dB] = $20\ log_{10} \frac{\sqrt{6}}{2}2^n \simeq 1.76 + 6.02n$
}
\item{Effective number of bits: $ENOB = \frac{SNR[dB]-1.76}{6.02}$
}
\end{enumerate}
\pagebreak

